MPC with Learned Residual Dynamics with Application on Omnidirectional MAVs

The growing field of aerial manipulation often relies on fully actuated or omnidirectional micro aerial vehicles (OMAVs) which can apply arbitrary forces and torques while in contact with the environment. Control methods are usually based on model-free approaches, separating a high-level wrench controller from an actuator allocation. If necessary, disturbances are rejected by online disturbance observers. However, while being general, this approach often produces sub-optimal control commands and cannot incorporate constraints given by the platform design. We present two model-based approaches to control OMAVs for the task of trajectory tracking while rejecting disturbances. The first one optimizes wrench commands and compensates model errors by a model learned from experimental data. The second one optimizes low-level actuator commands, allowing to exploit an allocation nullspace and to consider constraints given by the actuator hardware. The efficacy and real-time feasibility of both approaches is shown and evaluated in real-world experiments.

==> arxiv/01_introduction.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{INTRODUCTION}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Decomment only if accepted to RAL ----
\ifRAL
\IEEEPARstart{T}{he}
\else
%
The
\fi
%the introduction of interaction tasks as a new potential application for \acp{MAV} (particularly for \acp{OMAV}), the need arises to accurately track six \ac{DOF} trajectories at high speeds and at high levels of accuracy. The fact that such \acp{MAV} are complex to model is a driver to not only use previous knowledge from physics and first principles but also combine it with data-driven approaches in order to maximize performance. As there are many ways to formulate the given control problem, it is conducive that the formulation is general enough that it incorporates knowledge of actuator dynamics and constraints. \Ac{MPC} allows such a general formulation in that it gives the desired flexibility to explore alternative solutions to the same control problem, all the while depending on the choice of the cost function.
advancement of \acp{MAV} in the recent years has come with increasing focus on aerial physical interaction tasks. 
Investigations started with pick-and-place tasks,  continuing with contact-based inspection and push-and-slide operations \cite{Tognon2019,Bodie2019,Bodie2020,Nava2020,Tzoumanikas2020}, all the way to the manipulation of the environment \cite{Lee2020,Lee2021}. 
Tasks and applications involving aerial physical interaction are getting more complex year by year~\cite{9462539}.

%% PLATFORM DESIGNS:
Different platforms have been developed to cope with different challenges~\cite{2021-HamUsaSabStaTogFra}, some being generic for research or a broad spectrum of tasks, other being more specialized for certain applications.
Generally, aerial interaction requires a flying platform equipped with a manipulator that is designed to interact according to the desired task. This manipulator can be passive or actively controlled.  Depending on the task, the flying platform needs to meet certain requirements to compensate for wrenches (i.e., forces and torques) which arise during the interaction. While underactuated platforms are capable of compensating for some limited wrenches, \emph{fully actuated} and \emph{overactuated} platforms offer more freedom in this matter.
\emph{Fully actuated} platforms can compensate for any reaction wrenches that appear during interaction while \emph{overactuation} adds the benefit of redundancy. Furthermore, we refer to \emph{Omnidirectional} \acp{MAV} (OMAVs) as platforms that can generate thrust in any direction, providing sufficient lift force to hover in any possible orientation \cite{Hamandi2020}.
%A classification of different platform designs which takes into account the thrust and torque capabilities according to the geometry and actuators of a design has been done in \cite{Hamandi2020}.

However, full actuation and/or overactuation comes with new challenges and opportunities. First, the higher number of actuators gives potential for more unmodeled disturbances, e.g., through inaccurate thrust (or other actuator) mappings or airflow interferences. Second, it increases the complexity of finding optimal control inputs.
%% MOTIVATION:
Therefore, we intend to explore the possibilities of finding the optimal control inputs for performing a flight task while rejecting internal disturbances.

\begin{figure}[t]
    \input{figures/MPC_illustration.pdf_tex}
    % \includegraphics{figures/MPC_illustration.pdf}
    \caption{Illustration of MPC for trajectory tracking control.}\label{fig:mpc}
\end{figure}

%% CONTROL APPROACHES GENERAL/EXISTING SOLUTIONS:
%So far, control approaches mostly depend on the platform design, desired application (inspection, push-and-slide, manipulation), and available sensor data (force/torque sensor).
%Most commonly, controllers of \acp{MAV} can be divided into three parts:
Most common controllers of \acp{MAV} are divided into three parts:
\begin{enumerate*}[label=(\roman*)]
\item a high level controller for pose and/or force tracking (e.g., PD, impedance) which produces linear/angular acceleration commands,\label{item:tracking}
\item a wrench estimator to observe unmodeled disturbances, and\label{item:estimation}
\item an actuator allocation to convert high level commands into actuator commands\label{item:allocation}
\end{enumerate*}.
While this structure has proven to work reliably, it comes with a few drawbacks. First, the separation of a pose tracking controller and the actuator allocation does not allow to fully optimize the actuator commands for the execution of a desired task. Second, employing an online wrench estimator introduces time delays that can impair the actual flight performance.

The controller \ref{item:tracking} initially has often been implemented by a PD or impedance controller that generates acceleration commands based on the tracking errors. More recently, model-based optimal control approaches have been studied as well.
%% MPC in general (underactuated systems):
\Ac{MPC} can be specifically useful in situations where accurate and fast trajectory tracking is needed in the presence of actuator constraints and external disturbances~\cite{peric2021direct}. In this context, \cite{Hentzen2019} uses a \ac{MPC} on an underactuated quadrotor in strong wind gusts, comparing different Kalman filters for disturbance estimation. In this work the model based approach leads to higher position tracking accuracy than PID controllers. In a different work, \cite{Torrente2020} models aerodynamic disturbances by Gaussian Processes and fuses them in an \ac{MPC} to improve high-speed flight maneuvers with quadrotors. In \cite{Brunner2020}, we have presented an \ac{MPC}-based control framework for trajectory tracking of \acp{OMAV}. Optimizing on the wrench level, the individual rotor speed and tilt rotor inputs were then found through the same allocation process as presented in \cite{Bodie2019}. 
% The advantages and disadvantages of using linear vs. nonlinear MPC are presented in \cite{Kamel2017} with the application being trajectory tracking of underactuated \acp{MAV}.
% Additionally, \ac{MPC} offers the flexibility to add various objectives to the underlying optimization problem, as done in \cite{Falanga2018}, where the proposed framework takes into account action and perception objectives. 
% MPC also offers the ability to deal with input delays \cite{mpcDelay}.
% Challenge of MPC:
One difficulty of model-based approaches is their dependence on an accurate model of the system. If this is not known or contains unmodeled disturbances, these errors need to be either estimated online or compensated by an adaptive MPC.

%% Disturbance wrench estimation:
The wrench estimator \ref{item:estimation} can be implemented by a momentum-based observer (MBE) \cite{Ruggiero2014,Bodie2019}, or another estimation framework such as a Kalman filter \cite{Hentzen2019}.
The estimator usually accounts for both \emph{external} as well as \emph{internal} disturbances.  External disturbances can only be modeled to a certain degree (as they are caused by either interaction or unpredictable sources like wind gusts). Internal disturbances on the other hand are caused by unmodeled and unknown effects originating from the system itself. These can result from inaccurate hardware fabrication or complex aerodynamic effects.
A common disadvantage of using an online observer is the inherent time delay as it requires state observations in order to estimate the current disturbance. Therefore, the disturbances can also be learned offline based on experimental data and then applied during a flight. This approach has been applied in \cite{Zhang2020} by using Gaussian Processes to learn the wrench residuals.

%% ACTUATOR ALLOCATION
Lastly, the actuator allocation \ref{item:allocation} maps a wrench command into the actuator controls that will generate the desired wrench. It is determined by the particular actuation and geometry of the platform. According to the system, the actuator allocation problem can have a unique solution or, if the system is overactuated, an infinite number of solutions. This latter case can be exploited to achieve secondary objectives, like the minimization of energy or the optimization of actuation properties \cite{Ryll2015}.

% MOTIVATION:
%In this work, we explore the methods of how to use \ac{MPC} on an \ac{OMAV}. Specifically,  given by its tilt-rotor design, the \ac{OMAV} of our work is capable of a high level of overactuation and potential internal disturbances, leading to model errors.
%As we have learned from earlier work \cite{Brunner2020}, the dependency of \ac{MPC} on an accurate model representation of the real system can severely impact the flight performance. This is why we also look into how the control performance of an \ac{MPC} framework can be improved despite model uncertainties.
%An \ac{EKF}-based disturbance observer can help alleviate the influence of unmodeled disturbances but inherently causes a delayed reaction of the system.
%Additionally, applying \ac{MPC} on the wrench commands does not take into account the limitations of the actuators. Simultaneously, it is not able to fully exploit the available null space of the platform, therefore possibly not acting in the most effective way.

\subsection{Related works}
% MPC ON OVERACTUATED SYSTEMS
In order to cope with the above stated difficulties, various approaches have been investigated.
In \cite{Bicego2020}, the tracking controller and the allocation were in a single optimizer. This framework does not assume any linear model approximations nor does it depend on a cascaded control approach to decouple the translational and rotational dynamics of the rigid body. What is remarkable is the use of the derivatives of the individual propeller forces as control inputs which allows the direct translation of actual control inputs. Nevertheless, in the case of an \acp{OMAV} with actuated tilt angles, there is no explicit relationship between the generated individual forces and the actuator constraints.
\cite{Shawky2021} presented a \ac{NMPC} framework for overactuated MAVs with actively tiltable propellers.  Two optimizers were compared, namely Interior Point Optimization (through IPOPT) and Sequential Quadratic Programming (SQP) in CasADI through ACADO. However, the framework is only evaluated in simulations in Gazebo.

% LEARNING MPC
Also different methods to deal with the problem of uncertain or unknown model dynamics have been presented, such as \emph{adaptive MPC}, \emph{robust MPC} (e.g. Tube-MPC \cite{Chisci2001, Langson2004}), or \emph{learning-based} MPC.
A number of approaches exists to improve the MPC model by learning its true dynamics.
\cite{Hewing2020} gives an overview on how MPC performance can be improved through learning from recorded data. Accordingly, this can be achieved by following the following approaches:
\begin{enumerate*}[label=(\roman*)]
\item Learning the system dynamics, and/or\label{item:learning_dynamics}
\item learning the controller design, such as the optimal cost function or constraints\label{item:learning_design}.
\end{enumerate*}
\cite{Piga2019} followed the approach of \emph{Identification for control} (I4C), which aims to not minimize the output prediction errors (i.e. to fit the MPC model to the real system as closely as possible), but rather to find a model that optimizes the control performance in closed loop. In this approach, the MPC acts as an outer loop (i.e., as a \emph{reference governor}) that is based on a model of the inner loop, given by a fast PID controller. In this approach, closed loop experiments are repeated to find optimal control parameters through Bayesian Optimization.
% \cite{Terzi2018} learned prediction models from sampled input/output data. Using the `set-membership' approach.% Same for \cite{Terzi2018_2}.
As mentioned in \cite{Lorenzen2019}, ``stochastic and robust MPC are suitable for handling unmodeled dynamics and rapidly changing disturbances''. However, they are conservative and not appropriate for adapting to constant parameters.
% \cite{Adetola2009} employs parametric linear models with online parameter adaption. They assume that ``uncertainties in the system are due to static nonlinearities which can be expressed by unknown constant parameters''.
In \cite{Aswani2013} the concept of \ac{LBMPC} was introduced and applied on a quadrotor in \cite{Aswani2012}. \Ac{LBMPC} uses a so-called \emph{oracle} to learn the residual dynamics between a model and the true system dynamics. The oracle can be any linear or nonlinear parametric function whose parameters are adapted during the execution of the controller. In \cite{Aswani2012}, an \ac{EKF} is used for joint state and parameter estimation for a linear affine oracle.
Other approaches such as Iterative Learning MPC \cite{Bujarbaruah2018,Tamar2017} are restricted to repetitive tasks, in which the performance can be improved by adapting the control inputs by learning from earlier iterations.

\subsection{Contributions}
In this work, we explore the methods of how to use \ac{MPC} on an \ac{OMAV}. Specifically,  given by its tilt-rotor design, the \ac{OMAV} of our work is capable of a high level of overactuation and potential internal disturbances, leading to model errors.
We present the theory and experimental validation of an actuator-level NMPC that is able to generate real-time rotor speed and tilt angle commands for the task of trajectory tracking. Its knowledge of the actuator allocation allows to explore the actuation nullspace for an overactuated platform while respecting actuator constraints.
Furthermore, we show how internal model disturbances can be learned and applied through a simple linear model inside a wrench-level MPC.
Finally, we compare the performances of the different proposed approaches in various experiments.
% In our work we provide the following contributions:
% \begin{itemize}
% \item Theory and experimental validation of a actuator-level NMPC for trajectory tracking
% \item Linear regression of residual dynamics to augment the model in a wrench-level MPC framework
% \item Comparison of different combinations of control blocks in experiments
% \item Experimental evaluation
% \end{itemize}

%%%%%%%%%%%%%%%%%%
%% Story:
%%%%%%%%%%%%%%%%%%
% Develop optimal control for fully-actuated/overactuated vehicles
% Problems, difficulties:
% - Disturbances due to overactuation,
% - Actuator constraints, available dynamics dependent on tilt-angle configuration
% Therefore: Ideas:
% - Compare different MPC formulations
% - Develop method to compensate for disturbances
% Method:
% - MPC on wrench or on actuator level (WMPC, AMPC)
% - Disturbance prediction data-based, i.e., learned from datasets.
% - Difficulties: Disturbance model should be simple so that it can be used in MPC
% - Disturbance model cannot really be used in AMPC due to null space (i.e., due to overactuation)
% - Use a simple model to predict disturbances that can also be used within the MPC

% Vision, Motivation, Existing solutions, Challenge/gap, Our method, Results, (Menu)

==> arxiv/02_modeling.tex <==
\section{Modeling}
In this section we introduce the modeling of the system dynamics using Newton-Euler equations based on the following common assumptions: 
\begin{enumerate*}[label=(\roman*)]
\item The system is a single rigid body,\label{item:rigidbody}
\item mass and inertia matrix are constant,
\item the \ac{COM} coincides with the geometric center of the system, and
\item disturbance forces and moments can be reduced to a single wrench applied to the \ac{COM}.
\end{enumerate*}

\subsection{Notation}
We denote scalars by lowercase symbols, vectors $\vec{v}$ by lowercase bold symbols, and matrices $\mat{M}$ by uppercase bold symbols. If not specified differently, we use subscripts to indicate the frame of a vector $\f{W}\vec{v}$. To represent orientations, we use unit quaternions $\qB=\matrix{q_w & q_x & q_y & q_z}\transpose \in \nR{4}$, such that $\norm{\qB}=1$, as well as rotation matrices $\RB\in \SO(3)$.  Quaternions and rotation matrices can be used interchangeably, such that they act as vector transformations, i.e., $\f{W}\vec{v}=\vec{q}\otimes\f{B}\vec{v}\otimes\vec{q}^{-1}=\RB\f{B}\vec{v}$, where $\otimes$ represents the quaternion multiplication.

\subsection{Frame definitions}
We will refer to three reference frames: the inertial world frame $\frame{W} = \{\originW, \xW, \yW, \zW  \}$, the body frame $\frame{B} = \{\originB, \xB, \yB, \zB \}$ which is fixed to the geometric center of the \ac{OMAV}, and the local frame $\frame{L}=\{\originL, \xL, \yL, \zL \}$, which is obtained by a pure yaw rotation of the platform yaw angle from the world frame. $\origin_\star$ represents the center of the generic frame $\frame{\star}$, while $(\vX_\star,\vY_\star,\vZ_\star)$ represent its unit axes.
$\frame{W}$ is defined s.t. $\zW$ is aligned with the gravity vector $\gravity=\matrix{0 & 0 &-\SI{9.81}{\meter\per\square\second}}\transpose$.
\Cref{fig:frames} gives an overview of the frames used in this work.


% \begin{figure}[h]
% \includegraphics{figures/FrameView_labeled.pdf}\caption{Forces acting on the platform.}\label{fig:frames}
% \end{figure}

\begin{figure}[ht]
    \centering
    \def\svgwidth{0.9\columnwidth}
    \input{figures/FrameView_labeled_frames.pdf_tex}\caption{Frame definitions and forces/torques acting on the platform.}\label{fig:frames}
\end{figure}

\subsection{Rigid body dynamics}
%We model the \ac{OMAV} as a rigid body system by Newton-Euler mechanics.  
We define the system states as follows: The position of the \ac{COM} is given by $\pos\in\nR{3}$  in $\frame{W}$ and its velocity by $\vel\in\nR{3}$ in $\frame{B}$.  The attitude is expressed by the unit quaternion $\qB$ and the angular velocity by $\angVel\in\nR{3}$ in $\frame{B}$. The mass and inertia matrix are given by $\mass$ and $\inertia\in\nR{3\times 3}$, respectively.
We assume that we can reduce all forces and torques generated by the actuators to an individual actuator wrench acting on the \ac{COM}, expressed by $\actWrench=\matrix{\actForce\transpose & \actTorque\transpose}\transpose\in\nR{6}$, where $\actForce\in\nR{3}$ and $\actTorque\in\nR{3}$.
%
%Similarly, we define a residual wrench $\wrenchResidual=\matrix{\forceResidual\transpose,\torqueResidual\transpose}\transpose\in\nR{6}$ acting on the \ac{COM} to account for all unmodeled forces and torques.
%We assume that we can reduce all forces generated by the actuators to one force acting on the \ac{COM}, expressed by $\actForce\in\nR{3}$, and $\forceResidual\in\nR{3}$ as unmodeled residual forces. Similarly, the actuator torques are represented by $\actTorque\in\nR{3}$ and the di $\torqueResidual\in\nR{3}$. 
We can then write the dynamics as follows:
\begin{subequations}
\begin{align} 
    \dot\pos ={}& \RB\vel \\
    \dot{\qB} ={}& \frac{1}{2}\qB\otimes\begin{bmatrix} 0\\ \angVel\end{bmatrix} \\
    \dot\vel ={}& \mass^{-1}(\actForce + \forceResidual) + \RB\transpose\gravity - \angVel\times\vel\\
    \angAcc ={}& \inertia^{-1} \left(\actTorque + \torqueResidual - \angVel \times (\inertia\angVel)\right),\label{eq:angaccbody}%
\end{align}\label{eq:systemDynamics}%
\end{subequations}%
%
%\begin{align}
%\dot{\states}=\matrix{\posDot \\ \qBDot \\ \velDot \\ \angVelDot}
%\end{align}
where we considered a residual wrench $\wrenchResidual=\matrix{\forceResidual\transpose &\torqueResidual\transpose}\transpose\in\nR{6}$ acting on the \ac{COM}.
The residual (or disturbance) forces and torques $\forceResidual\in\nR{3}$ and $\torqueResidual\in\nR{3}$ account for all unmodeled effects, both internal and external, such as airflow interference (within rotor groups and between different rotor groups), hardware misalignments, or slightly different propeller characteristics. We assume that no further external or time-varying disturbances are present.
% In the course of this work we discuss methods to estimate these values.
Defining a state vector as $\states=\matrix{\pos\transpose & \qB\transpose & \vel\transpose & \angVel\transpose}\transpose$ we can then write the dynamic equations as
\begin{align}
    \dot\states=f_R(\states,\actWrench,\wrenchResidual).\label{eq:systemDynamicsShort}
\end{align}

\subsection{Allocation of actuator commands}
%As described earlier, we assume that we can reduce all actuator forces and torques to the lumped actuator wrench $\actWrench=\matrix{\actForce\transpose, \actTorque\transpose}\transpose\in\nR{6}$. 
%% QUESTION: Should we already use the parameters of our platform here? I.e. use 12 rotors and 6 arms instead of generic n_rotors, n_arms?

The \ac{OMAV} actuation can be described as follows: There are $\narms$ tiltable arms attached to the body core, with each arm carrying $\nrotperarm$ rotors, resulting in a total number of $\nrot=\narms\nrotperarm$ rotors.
The total actuator wrench $\actWrench$ is the result of the commanded rotor thrusts $\tprops\in\nR{\nrot}$ and the current tilt angle configuration, given by the tilt angles $\tiltAngles\in\nR{\narms}$. The geometry of the platform determines the relation between the actuator commands and the total actuator wrench $\actWrench$.
In the following we present a method for the \emph{actuator allocation} which computes actuator commands from a reference actuator wrench, i.e., $(\tiltAngles,\tprops)=f_{alloc}(\actWrench)$.
%This relation between the lumped wrench and the actuator commands is given by the geometry of the platform and is referred to as \emph{allocation}. 
\subsubsection*{Actuator allocation}
We define the vector $\thrustComponents(\tiltAngles,\tprops)\in\nR{2\nrot}$ that describes the vertical and lateral thrust components of each propeller in the body frame. We can then write the relation between $\actWrench$ and $\thrustComponents$ by a linear function:
%The relation between the actuator wrench and the individual actuator  commands
%The actuator forces and torques can be expressed as results of the tilt angles and rotor speeds. This correlation is given by the allocation:
\begin{subequations}
\begin{align}
    \actWrench(\tiltAngles,\tprops)&=\begin{bmatrix}
    \actForce\\
    \actTorque
    \end{bmatrix}=
    \allocationMatrix\thrustComponents(\tiltAngles,\tprops),\label{eq:allocation}\\
    % \text{ with }
    \thrustComponents(\tiltAngles,\tprops)&=\begin{bmatrix}
    f_{1,l}\\
    f_{1,v}\\
    \vdots\\
    f_{\nrot,l}\\
    f_{\nrot,v}
    \end{bmatrix}=\begin{bmatrix}
    \sin(\alpha_1)\tprop_1\\
    \cos(\alpha_1)\tprop_1\\
    \vdots\\
    \sin(\alpha_{\narms})\tprop_{\nrot}\\
    \cos(\alpha_{\narms})\tprop_{\nrot}
    \end{bmatrix}.\label{eq:extendedThrust}
\end{align}
\end{subequations}
Given this relation, the allocation matrix $\allocationMatrix\in\nR{6\times 2\nrot}$ is constant and can be obtained from the platform geometry.
%In order to compute the actuator commands $(\tiltAngles,\tprops)$ from a given actuator wrench $\actWrench$ we introduce the actuator allocation.
%We use \cref{eq:allocation} to compute optimal actuator commands from the actuator wrench.
In order to compute the actuator commands $\actInput\coloneqq\matrix{\tiltangles\transpose & \tprops\transpose}\transpose$ from a given actuator wrench $\actWrench$, we apply the Moore-Penrose Inverse:
\begin{subequations}
\begin{align}
\thrustComponents&=\allocationMatrix^\dagger\actWrench+\left(\eye{}-\allocationMatrix^\dagger\allocationMatrix\right)\vec{b}\label{eq:allocationGeneral}\\
\alpha_i&=\atantwo\left(\sum_j^{\nrotperarm} f_{j,l},\sum_j^{\nrotperarm} f_{j,v}\right)\quad\forall i=1\dots \narms\label{eq:alpha}\\
t_i&=\sqrt{f_{i,l}^2+f_{i,v}^2}\quad\forall i=1\dots \nrot.
\end{align}\label{eq:invAlloc}%
\end{subequations}%
If the system is overactuated, the vector $\vec{b}\in\nR{\nrot}$ can be used to find solutions in the nullspace of $\allocationMatrix$. For $\vec{b}=\bm{0}$ the norm of $\thrustComponents$ is minimized. Note that, due to the geometrical relation between $\thrustComponents$ and $\tprops$ in \cref{eq:extendedThrust}, the minimization of $\thrustComponents$ corresponds to a minimization of $\tprops$. We will refer to this solution as the \emph{minimum norm} or \emph{optimal allocation}, resulting in the optimal commands denoted by $\actInput^*=\matrix{\tiltangles^*{}\transpose & \tprops^*{}\transpose}\transpose$.
%For the remainder we will assume that $\vec{b}=0$.  

%Note that in \cref{eq:alpha} we use the sums of all generated thrusts for each arm to allow for multiple propellers fixed to an individual arm, such as coaxial rotors.

This procedure has the following properties:
\begin{enumerate*}[label=(\roman*)]
\item the norm of the resulting thrusts is minimized,\label{it:minnorm}
\item it is instantaneous,\label{it:instantaneous}
\item for $\vec{b}=\vec{0}$ the mapping $\actWrench\rightarrow(\tiltAngles^*,\tprops^*)$ is bijective, i.e.  for each $\actWrench$ there is a unique set of commands $(\tiltAngles^*,\tprops^*)$\label{it:bijective}
\end{enumerate*}.

While \ref{it:minnorm} and \ref{it:bijective} often provide advantages, \ref{it:instantaneous} can cause difficulties during fast motions. When $\actWrench$ changes rapidly, it can result in unfeasible fast changes of actuator commands. This can pose difficulties in the common separation of a high-level wrench generation controller and a low-level allocation.
In the following section, we will address this problem by introducing the allocation in the MPC formulation to impose cost and constraints on the actuator dynamics.


==> arxiv/03_method.tex <==
\section{Model Predictive Control Framework}

In this section, we present two different model-based controllers for the task of free flight trajectory tracking with an overactuated aerial vehicle.
%formulations which we will solve with the same receding horizon optimal control problem.% Both formulations are based on the rigid body dynamics \cref{eq:systemDynamics}.
Both methods are based on the same formalisms to model the system dynamics but differ in the level of detail to which the models are embedded and how residual wrenches are handled. Specifically, the first approach optimizes wrench commands and uses a default allocation, while the second approach operates on the actuator level. We refer to these two proposed methods as \ac{WMPC} and \ac{AMPC}, respectively.
Both controllers rely on residual wrench estimates to account for otherwise unmodeled disturbances. These estimates can either be provided by an online estimator (EKF) or by a Residual Dynamics Model (RDM).
\Cref{fig:wmpc_ampc_diagram} illustrates the two different methods in a control block diagram and \cref{tab:comparison} compares the similarities and differences between the two methods.
% We first introduce a general formulation of MPC and then apply this theory on the two different approaches.
\begin{table*}[t!]
    \centering
    \begin{tabular}{c c c}
        \hline
         & \textbf{WMPC} & \textbf{AMPC}\\
        \hline 
        {Output} & Actuator wrench derivative $\actWrenchDot$ & Actuator commands derivative $\drotorSpeeds, \dtiltAngles$\\
        % \hline 
        {Allocation} & Minimum norm allocation after MPC & Implicitly in MPC\\
        % \hline 
        {Disturbance compensation} & Disturbance observer or model-based & Disturbance observer\\
        \hline 
    \end{tabular}\caption{Comparison of WMPC and AMPC.}
    \label{tab:comparison}
\end{table*}

% \begin{figure}[ht]
% \includegraphics[width=\columnwidth]{figures/WMPC_blockdiagram.pdf}\caption{WMPC  block diagram.}\label{fig:wmpc_diagram}
% \end{figure}

% \begin{figure}[ht]
%     \includegraphics[width=\columnwidth]{figures/AMPC_blockdiagram.pdf}\caption{AMPC  block diagram.}\label{fig:ampc_diagram}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \input{figures/wmpc_diagram_latex.tikz}\caption{WMPC  block diagram. The wrench residual $\wrenchResidualModel$ can be applied either in the WMPC formulation (\emph{In-MPC}, dashed) or added as a correcting feedforward-term (\emph{Post-MPC}, dotted).}\label{fig:wmpc_diagram}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \input{figures/ampc_diagram_latex.tikz}\caption{AMPC  block diagram.}\label{fig:ampc_diagram}
% \end{figure}

\begin{figure}[ht]
    \centering
    \input{figures/wmpc_ampc_diagram_latex.tikz}\vspace{0.2cm}
    \caption{Control block diagram. Either the AMPC alone or the combination of WMPC and allocation can compute the actuator controls. The wrench residual $\wrenchResidualModel$ can be applied either directly in the WMPC formulation (\emph{In-MPC}, dashed) or added as a correcting feedforward-term (\emph{Post-MPC}, dotted). For AMPC, only residuals from the EKF can be applied.}\label{fig:wmpc_ampc_diagram}
\end{figure}


%\begin{itemize}
%    \item MPC on wrench level vs. actuator level
%    \item Linear model learning
%    \item Linear model in the MPC optimization
%\end{itemize}

\subsection{MPC formulation}
We first introduce a general formulation of the MPC problem.  To this end, we define the state vector as $\states\in\stateSpace\subseteq\nR{\nstates}$ and the input vector as $\inputs\in\inputSpace\subseteq\nR{\ninputs}$. 
We further assume that states and control inputs are constrained by the polytopes $\stateSpace$ and $\inputSpace$.
The system is subject to its dynamics $\dot\states=\vec{f}(\states,\inputs)$, discretized as $\states_{k+1}=\discreteDynamics(\states_k,\inputs_k)$.
We also define the stage cost $\stageCost(\states,\states_{\des})$ and terminal cost $\stageCost_N(\states_N,\states_{\des,N})$.
The discrete-time MPC problem is then formulated as the minimization of a cost function over a finite time horizon of $N$ steps:
%Generally, MPC solves an optimization problem in a receding horizon fashion by minimizing a cost function $\mathcal{L}(\states,\inputs)$ over an input sequence of $N$ steps, i.e.
%We define the state vector as $\states\in\nR{n}$ and the input vector as $\inputs\in\nR{m}$. We further assume that the states $\states\in\stateSpace$ and the control inputs $\inputs\in\inputSpace$ are constrained by the polytopes $\stateSpace$ and $\inputSpace$.
%The system dynamics can then be expressed by
%\begin{align}
%\dot\states = f(\states,\inputs) + g(\states,\inputs),
%\end{align}
%where $f(\states,\inputs)$ describes the dynamics modeled by first principles and $g(\states,\inputs)$ the residual (unmodeled) dynamics.

% In general, we define the receding horizon optimal control problem as follows:
\begin{subequations}
\begin{align}
\begin{split}
\min_{\inputs}\sum_{k=0}^{N-1}\biggl(\norm{\stageCost(\states_k,\states_{\des,k}&)}^2_{\mpcStateWeights}+\norm{\inputs_k}^2_{\mat{R}}\biggr)\\
&\quad+\norm{\stageCost_N(\states_N,\states_{\des,N})}^2_{\mpcStateWeights_N}
\end{split}\label{eq:mpc_optimization}\\
\begin{split}
\text{subject to}\quad&\states_k\in\stateSpace, \inputs_k\in\inputSpace\\
&\states_{k+1}=\discreteDynamics(\states_k,\inputs_k)\\
&\states_0=\states(t).
\end{split}\label{eq:mpc_subject}%
\end{align}\label{eq:mpc}%
\end{subequations}%
The matrices $\mpcStateWeights,\ \mpcStateWeights_N\in\nR{\nstates\times \nstates}$ and $\mpcInputWeights\in\nR{\ninputs\times \ninputs}$ represent the state, terminal state, and input cost matrices, respectively.
For the remainder of this section we present the details and differences of the two approaches and how \cref{eq:mpc} is adapted accordingly.
%&\Delta\force_k = \Delta\hat{\force}(t) \\
%&\Delta\torque_k = \Delta\hat{\torque}(t)
\subsection{State and input vectors for different model formulations}
For the two formulations of the \ac{WMPC} and \ac{AMPC} we use different definitions of state and input vectors.
\subsubsection{Wrench-MPC}
In the case of \ac{WMPC} we define the state vector to comprise both the \ac{OMAV} and the wrench states. The modeling of the state dynamics is equal to the rigid body dynamics in \cref{eq:systemDynamicsShort}.
\begin{subequations}
\begin{align}
\states_W&=\matrix{\actWrench\transpose & \pos\transpose & \vel\transpose & \qB\transpose & \angVel\transpose}\transpose\in\nR{19} \\
\inputs_W&=\actWrenchDot\in\nR{6}.
\end{align}
\end{subequations}
\subsubsection{Actuator-MPC}
While the system dynamics in \ac{AMPC} are described equivalently to \ac{WMPC}, we include the actuator commands $\actInput=\matrix{\tiltangles\transpose & \tprops\transpose}\transpose$ in the state as well as the allocation \cref{eq:allocation} in the MPC system dynamics.
\begin{subequations}
\begin{align}
\states_A&=\matrix{\tiltangles\transpose & \tprops\transpose & \pos\transpose & \vel\transpose & \qB\transpose & \angVel\transpose}\transpose\in\nR{31} \\
\inputs_A&=\matrix{\tiltanglesdot\transpose & \tpropsdot\transpose}\transpose = \actInputDot \in\nR{18}.
\end{align}
\end{subequations}
By including the actuator commands in the model, the MPC does not rely on the allocation procedure \cref{eq:invAlloc}, thus allowing a larger exploration space of possible solutions. Additionally, we can impose constraints on actuator velocities and ensure continuity of the commands.

\subsection{Cost vector}
The cost vector $\stageCost(\states,\states_{\des})$ is designed slightly different for the two different approaches of \ac{WMPC} and \ac{AMPC}. Both have in common that a reference trajectory is to be tracked, given by the time dependent variables $\pos_\des,\vel_\des,\qB_\des,\angVel_\des$.
\subsubsection{Wrench-MPC}
We employ a common definition of tracking errors to write the cost vector:
\begin{align}
\stageCost(\states_k,\states_{\desk})=\matrix{\pos_k-\pos_{\desk} \\ \vel_k-\vel_{\desk} \\ \qErrk \\ \angVel_k-\RB \transpose \RBdes \angVel_{\desk}},% \\ \dot\vel_k \\ \dot\angVel_k}
\end{align}
with $\qErr\in\nR{3}$ as the vector that describes the rotation error between $\qB$ and $\qB_\des$, such that
\begin{equation}
% \Delta\qB=\qB^{-1}\qB_\des \eqqcolon \matrix{0\\ \qErr},\quad\qErr\in\nR{3}
\qB_\des=\qB\otimes\Delta\qB,\quad \Delta\qB\coloneqq \matrix{1 \\ \qErr}.
\end{equation}
\subsubsection{Actuator-MPC}
The actuator-based MPC further includes the tilt angles and propeller thrusts as state variables:
\begin{align}
    \stageCost(\states_k,\inputs_k)=\matrix{\pos_k-\pos_{\desk} \\ \vel_k-\vel_{\desk} \\ \qErrk \\ \angVel_k-\RB \transpose \RBdes \angVel_{\desk} \\ \tiltAngles_k-\tiltAngles_{\desk} \\ \tprops_k-\tprops_{\desk}}.
\end{align}
Generally, we aim to allow the actuator dynamics to evolve as freely as possible. There are different possibilities to penalize these states.
% Penalizing the thrust in general would lead to non-optimal trajectory tracking, since this would require to find a tradeoff between tracking performance and minimum thrust.
% Not penalizing the tilt angles $\tiltAngles$ would allow full exploration of the allocation nullspace, but could easily lead to local minima.
Not penalizing the actuator states would allow the largest exploration freedom but would could also lead to long optimization times of the MPC.
Therefore, we chose to penalize the deviation of the actuator commands from the minimum norm commands $(\tiltAngles^*,\tprops^*)$:
\begin{subequations}
    \begin{align}
        \tiltAngles_{\desk} &= \tiltAngles^*_t\\
        \tprops_{\desk} &= \tprops^*_t.
    \end{align}
\end{subequations}
Tuning of the weight matrix $\mpcStateWeights$ then allows to give more or less range in deviating from the optimal allocation.
The minimum norm commands $(\tiltAngles^*_t,\tprops^*_t)$ are obtained assuming static hover, i.e., only exerting the force required to hold the platform weight in the current attitude.


\subsection{Constraints}
In order to obtain smooth control inputs and to account for unmodeled dynamic effects, we can employ hard constraints on any of the states and inputs.
\subsubsection{\ac{WMPC}}
In the case of WMPC, we constrain the total actuator wrench $\actWrench$ and its derivative $\actWrenchDot$. This allows us to ensure that both the total wrench and the wrench rate remain in feasible bounds. Note that employing constraints on the wrench rate implicitly constrains the actuator rates due to the relation in \cref{eq:allocation}.
\begin{subequations}
    \begin{align}
    % -d\actForceConstraint \leq df \leq d\actForceConstraint\\
    % -d\actTorqueConstraint \leq d\actTorque \leq d\actTorqueConstraint\\
    % -\actForceConstraint \leq \actForce \leq \actForceConstraint\\
    % -\actTorqueConstraint \leq \actTorque \leq \actTorqueConstraint
    -\actWrenchDotConstraint \leq \actWrenchDot \leq \actWrenchDotConstraint\\
    -\actWrenchConstraint \leq \actWrench \leq \actWrenchConstraint
    \end{align}
\end{subequations}

\subsubsection{\ac{AMPC}}
One major advantage of AMPC is the possibility to constrain actuator commands directly. Therefore, we employ hard constraints on the thrusts, the thrust rates, and the tilt angle rates:
\begin{subequations}
    \begin{align}
        \tpropsMin \leq {}&\tprops \leq \tpropsMax\\
        -\tpropsdot_{max} \leq {}&\tpropsdot \leq \tpropsdot_{max}\\
        -\tiltanglesdot_{max} \leq {}&\tiltanglesdot \leq \tiltanglesdot_{max}
    \end{align}
\end{subequations}

\subsection{Optimal problem result}
Each MPC iteration of solving \cref{eq:mpc} returns a sequence of optimal inputs $U=\left[\inputs_0^*,\dots,\inputs_N^*\right]$ and associated states $X=\left[\states_0^*,\dots,\states_N^*\right]$. We use this state sequence to extract the optimal inputs and apply them as control inputs to the system --- either $\actWrench$ in the case of WMPC or $\actInput$ in the case of AMPC.


==> arxiv/04_learning.tex <==
\section{Compensation for disturbances}
We identify model mismatches as a main cause that leads to non-optimal tracking of reference trajectories. Therefore, we introduce two methods to tackle this challenge: \begin{enumerate*}[label=(\roman*)]
    \item an EKF-based disturbance observer, and
    \item a linear model that predicts disturbance wrenches based on experimental data.
\end{enumerate*}
Both methods intend to predict the residual wrench $\wrenchResidual=\matrix{\forceResidual\transpose & \torqueResidual\transpose}\transpose$ for each flight configuration.

\subsection{Disturbance observer}
We employ an \ac{EKF} to estimate the disturbance force and torque in real time. %We have previously applied this approach in \cite{Brunner2020}.
We assume that most disturbances originate from internal model errors, e.g., from interfering air flows, inaccurate rotor-speed/thrust mapping, or misaligned tilt arms. Furthermore, we assume that these internal errors are independent of the platform yaw angle $\psi$.
Therefore, we estimate the disturbance force in the local frame $\frame{L}$, which is obtained by a pure yaw rotation of the platform yaw angle from the world frame, i.e., $\rotMat_L=\rotMat_z(\psi)$.
We use the following state vector $\stateEst\in\nR{19}$, inputs $\ekfInputs\in\nR{6}$, and measurements $\ekfMeasurements\in\nR{7}$:
\begin{align}
\stateEst=\matrix{\posEst\\ \velEst \\ \qBEst \\ \angVelEst \\ \distForceEst \\ \distTorqueEst},\quad\ekfInputs=\matrix{\actForce\\ \actTorque},\quad\ekfMeasurements=\matrix{\posMeas\\ \qBMeas}.
\end{align}
The formulation of linear and rotational dynamics is equal to \cref{eq:systemDynamicsShort}, while the evolution of the disturbance force and torque is assumed to be constant, i.e.
\begin{subequations}
\begin{align}
\ddt\distForceEst&=\processNoise_{\distForceEst}\\
\ddt\distTorqueEst&=\processNoise_{\distTorqueEst},
\end{align}
\end{subequations}
where $\processNoise_{\distForceEst}\sim\mathcal{N}(\zeros,\mat{\Sigma}_f),\ \processNoise_{\distTorqueEst}\sim\mathcal{N}(\zeros,\mat{\Sigma}_\tau)$ represent the process noise, respectively.
%
We obtain the disturbance force in the body frame by the following rotation:
\begin{align}
    \forceResidualEst&=\RB\transpose\rotMat_L \distForceEst.
\end{align}
The force and torque disturbance estimates are directly employed in the dynamic model of the MPC formulation, specifically in \cref{eq:systemDynamicsShort}.

\subsection{Residual Dynamics Model (RDM)}
The above introduced method of estimating disturbances online comes with the downside of being time-dependent and, therefore, can introduce time delays. Therefore, we now present another method which relies on estimating the internal disturbances based on a model which is trained by experimental data.
To this end, we approximate the true residual wrench $\wrenchResidual$ with a linear model $\wrenchResidualModel=f(\features)$, with $\features$ as a feature vector.
We follow a similar approach as in \cite{Aswani2012} with the difference of learning the parametric uncertainties offline rather than in-flight. This has the advantage that the parameters are not estimated online which could lead to unpredictable and inconsistent flight behavior.

\subsubsection{Model definition}
We use a feature vector $\features\in\nR{\nfeatures}$, to create a linear affine relationship between a set of $\nfeatures$ features and the residual wrench:
%We use a linear affine function to approximate the residual dynamics:
\begin{align}
\wrenchResidualModel(\features)=\modelMatrix\features,
\end{align}
%We look to model the residual dynamics linearly in a set of features so that it can efficiently be embedded in an MPC framework. We define the set of features as $\features\in\nR{\nfeatures}$ and want to find a linear relationship
where $\modelMatrix\in\nR{6\times \nfeatures}$ is a matrix that maps from features to wrench residuals.
The choice of a simple linear model allows us to employ it in the MPC framework while maintaining a low computational complexity.

% Our goal is to find a matrix $\modelMatrix$ and vector $\outputsMean$ such that $\outputs(\features)$ approximates $\wrenchResidual(\features)$.

%Since we want to find a model for the residual dynamics, we set the output to the stacked residual forces and torques:
%\begin{equation}
%\outputs=\matrix{\forceResidual \\ \torqueResidual}
%\end{equation}

\subsubsection{Feature selection}
Selecting an appropriate set of features is important to capture relationships between available data and perceived dynamic residuals while keeping the mathematical complexity low.
We will present our selection of features in the experimental section \ref{sec:wmpcmodel}.
% Essentially, all data that is available to the controller can be used as features. In doing that, we want to avoid selecting redundant data as features.  Additionally, we want to cover a largest possible area of the state space with a minimal set of features. Minimizing the number of features will also help reduce the complexity of the MPC optimization.
% We propose the following features that affect the dynamic residuals:
% \begin{itemize}
% \item Commanded wrench
% \item Attitude (with exception of the yaw angle)
% \item Linear and angular velocity
% \end{itemize}

% We do not propose the following features:
% \begin{itemize}
% \item Position
% \item Actuator commands (such as tilt angles and rotor speeds), as they can be directly inferred from the commanded force and torque commands (\red{depending on the MPC formulation})
% \end{itemize}

%\begin{itemize}
%    \item Feature selection
%    \item Output computation (i.e. model error)
%\end{itemize}


==> arxiv/05_training.tex <==
\subsubsection{Training}
In this section we describe the process of finding the model matrix $\modelMatrix$ %and vector $\outputsMean$
for an optimal performance when employing the learned model in the control loop.

% As described earlier, we compute the parametric model offline based on recorded flight data of the real system.

Given a dataset of $\nsamples$ experimentally recorded residual wrenches $\wrenchResidual_{m,i}$ and features $\features_i,\ i\in{1,\dots,\nsamples}$ we want to find $\modelMatrix$ s.t.
\begin{align}
    \modelMatrix&=\argmin_{\modelMatrix}\sum_{i=1}^{\nsamples}\trainError{}_{,i}\\
    \trainError{}_{,i}&=\norm{\modelMatrix\features{}_i-\wrenchResidualMeasured{}_{,i}}.
\end{align}
\subsubsection{Computation of dynamics residuals}
% \begin{align}
%  \forceResidual &= - \actForce + \mass(\dot\vel - \RB\transpose\gravity + \angVel\times\vel)  \\
%  \torqueResidual &= - \actTorque + \inertia(\angAcc + \angVel \times (\inertia\angVel))
% \end{align}
We use linear acceleration and angular velocity data obtained from an onboard \ac{IMU}, $\imuLinAccMeas$ and $\imuAngAccMeas$, respectively, to compute the residuals from recorded training datasets. The recorded angular velocity $\imuAngVel$ is differentiated numerically to obtain the angular acceleration $\imuAngAcc$.
% \begin{align}
% \imuLinAccMeas &= \linAcc + \imuLinBias + \imuLinNoise - \RB\transpose\gravity \\
% &= \dot\vel + \angVel\times \vel- \RB\transpose\gravity  + \imuLinBias + \imuLinNoise\\
% \imuAngVel &= \angVel + \imuAngVelBias + \imuAngVelNoise
% \end{align}

Furthermore, we employ MSF \cite{Lynen2013} to correct the linear acceleration measurements for the IMU bias.

We can then compute the wrench residuals from the measured accelerations as
\begin{align}
\wrenchResidualMeasured=\matrix{\forceResidualMeasured \\ \torqueResidualMeasured}=\matrix{\mass\imuLinAccMeas-\actForce \\ \inertia\imuAngAcc-\actTorque}
\end{align}

In order to compute the model parameters we use ridge regression to minimize the training error. We train each row of the model matrix individually. Let us define the feature matrix for $\nsamples$ samples as $\featureMatrix\in\nR{\nsamples\times\nfeatures}$ and the vector of measured residuals for the $i$-th component of the wrench $\vec{y}_i$:
\begin{align}
\featureMatrix=\matrix{\features_0 & 1\\ \features_1 & 1 \\ \vdots \\ \features_{\nsamples-1} & 1},\quad \vec{y}_i=\matrix{\wrenchResidual_{i,0}\\ \wrenchResidual_{i,1}\\ \vdots\\ \wrenchResidual_{i,\nsamples-1}},\quad\modelMatrix=\matrix{\vec{c}_0 \\\vec{c}_1 \\ \vdots \\ \vec{c}_5},
\end{align}
where $\vec{c}_i\in\nR{1\times \nfeatures}$ represents the $i$-th row of the model matrix. 
We can then find the model coefficients for each wrench component individually:
\begin{align}
\vec{c}_i=\argmin_{\vec{c}_i} \norm{\vec{y}_i-\featureMatrix\vec{c}_i\transpose}+\regParam\norm{\vec{c}_i},\quad i\in\{0,\dots,5\}.\label{eq:ridgeRegression}
\end{align}
Note that \cref{eq:ridgeRegression} is a ridge regression with $\regParam$ as the regularization parameter that helps avoid overfitting to the training data.

% \begin{align}
% \trainError&=\wrenchResidual-\wrenchResidualMeasured=\modelMatrix%\features-\wrenchResidualMeasured
% \end{align}
% where $\params_i=\matrix{\modelMatrix_{i,:},\outputsMean_i}$.
% THIS NEEDS TO BE FIXED.

% \red{
% \begin{itemize}
%     \item Data recording
%     \item Filtering
%     \item Accelerometer bias removal
%     \item Influence of IMU position offset w.r.t. geometric center
%     \item Normalization
%     \item Outlier filtering
%     \item Clustering, with or without normalization
%     \item Performance of different features and models on 
% \end{itemize}
% }

\subsubsection{Application of the residuals in the control loop}
Generally, we only employ the residual model in the WMPC formulation only and not in AMPC. %where we use the minimum-norm solution of the allocation to generate the actuator commands.
This is because the allocation nullspace exploitation in AMPC can result in various different actuator commands $\actInput$ for the same states, leading to different wrench residuals as a consequence and making a parametric model infeasible. % (non-injectivity of wrench to actuator commands)

Within WMPC, we investigate two different methods of applying the residual model in the control framework. 
\paragraph{In-MPC} In this approach, the model is implemented in the state dynamics of the MPC formulation. This allows the controller to respect the residual dynamics while computing an optimal input trajectory.
\paragraph{Post-MPC} In this approach, the MPC is agnostic of any model inaccuracies. Instead, the resulting optimal wrench commands $\actWrench^*$ are corrected after the MPC optimization.

% \red{
% \subsection{Discussion of training data}
% \begin{itemize}
%     \item Appropriateness for specific trajectory
%     \item Linearity around setpoint / reference trajectory
%     \item Importance of injective mapping of allocation -- requirement for wrench level MPC?
% \end{itemize}
% }

\subsection{Discussion}
The first approach of employing an EKF-based disturbance observer has the advantage of being simple to implement while being able to adapt to most disturbances. On the other hand, it introduces a time delay into the system as it requires sensor measurements to adapt its estimates.% Furthermore, the EKF can be used for both WMPC and AMPC, model based only for WMPC because it requires a consistent allocation.

The model-based approach can be instantly applied in the controller framework, not adding any time delays. However, it requires a rich dataset upon which the model parameters can be fit. Additionally, selecting the correct features and a reasonable regularization parameter is not straight forward. Because of its linear formulation it can also only cover a limited area around a specific operating point.




==> arxiv/06_experiments.tex <==
\section{Experimental validation}

\subsection{Implementation}

\subsubsection{Flying platform}
We perform all experiments on our custom built \ac{OMAV}. This platform is designed with 6 arms equally spaced around its body center. Each arm can be tilted individually by a Dynamixel XL430-W250-T servo. At the end of each arm a double rotor group, containing two KDE2315XF-885 motors with counter rotating 9x\SI{4.5}{in} propellers is mounted.  The counter rotation of each rotor group minimizes the net torque of each arm, but the exact influence of the airflow interferences is unknown.
The entire system is powered by a single \SI{7000}{\milli\amperehour} battery. Fully prepared for a flight its mass is $\SI{4.36}{\kilo\gram}$.

\subsubsection{Software}
The entire controller is implemented in ROS on an Intel NUC that is mounted on the platform.  Reference trajectories are transmitted via WiFi from an offboard computer.
The onboard computer runs the MPC solver and publishes either wrench or actuator commands (according to WMPC or AMPC), which are forwarded to a Pixhawk flight controller. For WMPC, the flight controller computes the optimal actuator commands and sends them to the actuators, while for AMPC it solely passes the commands through to the actuators.

The MPC optimizer is implemented using the ACADO framework. The system dynamics are discretized through direct multiple shooting and solved through an Implicit Runge Kutta method (Gauss-Legendre integrator of order 6). We use qpOASES as the QP solver.
%% Literature background on implementation of MPC:
% \cite{Shawky2021} compared two optimizers for MPC on an \ac{OMAV}, namely Interior Point Optimization (through IPOPT) and Sequential Quadratic Programming (SQP) in CasADI through ACADO. However, the framework is only evaluated in simulations in Gazebo.

\subsection{Model for WMPC}\label{sec:wmpcmodel}
We have tested different feature sets for the model.  For the experiments we used a set made up from the commanded wrench and the roll and pitch angle, encoded by the 3rd row of the rotation matrix $\RB$, resulting in 9 features:
\begin{equation}
\features=\matrix{\actWrench\transpose & -\sin(\theta) & \cos(\theta)\sin(\phi) & \cos(\theta)\cos(\phi)}\transpose.
\end{equation}
It turned out that the regularization parameter $\regParam$ is an essential tuning parameter for the closed loop stability.
Low values of $\regParam$ lead to a better model fit to the training data,  but also to high residual predictions, resulting in strong countersteering and increasing instabilities. We therefore converged to choosing a high value of $\regParam=\SI{1e5}{}$.

We recorded a training dataset which consists of two trajectories: the first one containing pure pitching and rolling motions of with a duration of \SI{167}{\second} and the second one tracking out a horizontal square, lasting \SI{178}{\second}.
This dataset therefore contains both angular as well as linear acceleration data.
The results of the model fit are presented in \cref{fig:modelErrors} and \cref{tab:modelErrors}.
Both the table and the figure show the RMSE of the training data, i.e. of $\trainError$. It can be seen that the model is able to compensate especially static offsets in both force and torque.

% \begin{figure}[h]
% \includegraphics[width=\columnwidth]{plots/3639c3dab7_Model_errors_per_axis.pdf}\caption{Model fit errors.}\label{fig:modelErrors}
% \end{figure}
\begin{figure}[t]
    \includegraphics[width=\columnwidth]{plots/3639c3dab7_Model_errors_per_actuation.pdf}\caption{Model fit errors for residual forces and torques. The blue violinplots represent the raw residual data $\wrenchResidualMeasured{}_{,i}$ and the orange violinplots represent the residuals after fitting $\trainError{}_{,i}$.}\label{fig:modelErrors}
\end{figure}

\begin{table}[t!]
\centering
\begin{tabular}{c c c}
\hline 
 & RMSE force [\si{\newton}] & RMSE torque [\si{\newton\meter}] \\ 
\hline 
Raw & $1.444\pm 0.867$  & $0.347\pm 0.147$ \\
Model ($\regParam=\SI{1e5}{}$) & $1.144\pm 0.669$ & $0.177\pm 0.115$ \\
Exact Model ($\regParam=0$) & $0.959\pm 0.517$ & $0.087\pm 0.057$ \\
\hline
\end{tabular}\caption{Force and torque RMSE and std. deviations of raw data and after model fit.}
\label{tab:modelErrors}
\end{table}

\subsection{Experiments}
The presented building blocks of WMPC/AMPC and disturbance observer/parametric model are combined in different ways to evaluate their performances in real-world experiments. 

Specifically, we aim to analyze the following characteristics: \begin{enumerate*}[label=(\roman*)]
    \item Position and attitude tracking performance, and
    \item velocity of actuator commands as well as nullspace exploitation of the AMPC.
\end{enumerate*}

% WMPC and AMPC are evaluated separately, focusing on different effects.

We evaluate the controllers by comparing their capabilities to track given 6-\ac{DOF} trajectories in free space with an \ac{OMAV}.
We use four different trajectories and different velocities to evaluate the tracking performance: \begin{enumerate*}[label=(\roman*)]
\item square trajectory: horizontal square with \SI{1}{\meter} leg length and reference velocities up to \SI{3}{\meter\per\second},
\item attitude trajectory: pure pitching and rolling up to \SI{45}{\degree} while hovering at a fixed position with a duration of \SI{27}{\second},
\item lemniscate trajectory: combined position and attitude trajectory tracking a bent lemniscate with a two possible speeds (slow: \SI{15}{\second} duration, up to \SI{0.9}{\meter\per\second} and fast: \SI{5.5}{\second}, up to \SI{2.9}{\meter\per\second}), as presented in \cref{fig:lemniscate}, and
\item horizontal step responses along the $x$-axis with \SI{1}{\meter} length.
\end{enumerate*}
We compute the attitude errors as euler angles of the actual attitude w.r.t. the \emph{reference} attitude. That way, we avoid large or distorted angle errors at large roll/pitch angles. Accordingly, the attitude RMSE is the RMSE of the error euler angles.

\Cref{tab:settings} presents the values of the most important tuning parameters. Note that the horizon length for AMPC is shorter than for WMPC in order to keep the computational complexity low. In both cases we use a time discretization of \SI{50}{\milli\second}, resulting in time horizons of \SI{1}{\second} for WMPC and \SI{0.5}{\second} for AMPC, respectively.

\begin{figure}[t]
    % \centering
    % \begin{subfigure}{.5\columnwidth}
        \centering
        % \includegraphics[width=\linewidth]{plots/14_3D_reference_trajectory_eight.pdf}
        \includegraphics{plots/14_3D_reference_trajectory_eight.pdf}
        \caption{Bent lemniscate trajectory. Note that this trajectory also involves pitch angles up to \SI{30}{\degree}.}\label{fig:lemniscate}
    % \end{subfigure}%
    % \begin{subfigure}{.5\columnwidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{plots/12_3D_reference_trajectory_square.pdf}
    %     \caption{Horizontal square trajectory.}\label{fig:square}
    % \end{subfigure}
    % \caption{Bent lemniscate (left) and square trajectory (right).}
\end{figure}


%\begin{table*}[t!]
%\centering
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline 
%• & No d/o & EKF & Residual model in MPC & Residual Model post MPC & EKF+Res. Model \\ 
%\hline 
%MPC on wrench & • & • & • & • & \\ 
%\hline 
%MPC on actuators & • & • & n/a & n/a & \\ 
%\hline 
%\end{tabular}\caption{Possible combinations of building blocks.}
%\label{tab:combinations}
%\end{table*}

\begin{table}[t!]
    \centering
    \begin{tabular}{c c c}
    \hline 
    Parameter & WMPC & AMPC \\ 
    \hline 
    $N$ & 20 & 10 \\
    $\Delta t$ & \SI{0.05}{\second} & \SI{0.05}{\second}\\
    $\actForceConstraint$ & \SI{20}{\newton} & \SI{20}{\newton} \\
    $\actTorqueConstraint$ & \SI{20}{\newton\meter} & \SI{20}{\newton\meter} \\
    $\tiltanglesdot_{max}$ & n/a & \SI{10}{\radian\per\second}\\
    $\tprops_{max}$ & n/a & \SI{16}{\newton}\\
    $\tprops_{min}$ & n/a & \SI{0.1}{\newton}\\
    $\tpropsdot_{max}$ & n/a & \SI{29}{\newton\per\second}\\
    \hline 
    \end{tabular}\caption{Control parameters for WMPC and AMPC.}
    \label{tab:settings}
\end{table}
% Notes: In cpp, we use omega_squared for the constraints.
% rotor_force_constant (cF): 7.2e-6
% omega_sq_dot_max = 4e6 --> 28.8 N/s
% omega_sq_max = 2.25e6 --> 16.2 N
% omega_sq_min = 1e4 --> 0.072 N

\subsection{WMPC}
We evaluate the different variations of WMPC (i.e., no correction for disturbances, residual model in- or post-MPC, or online disturbance observer) by tracking different trajectories. Specifically, we focus on the influence of the disturbances on the tracking performance, and how well these can be compensated by the linear model approach.
\Cref{tab:trackingWMPC} gives an overview of the RMSE of each experiment. It shows that in most cases the Post-MPC variant outperforms all other configurations by a small margin. This is also highlighted in \cref{fig:wmpc_te_violin}, where we show the pose tracking errors only for the attitude trajectory in different configurations.

\begin{table}[t!]
\centering
\begin{tabular}{c|c|c|c|c}
\hline 
Position err. [\si{\meter}] & N/c & In-MPC & Post-MPC & D/o \\ 
\hline 
Squares & 0.198 & 0.172 & \textbf{0.150} & - \\
Attitude trajectory & 0.139 & \textbf{0.088} & 0.104 & 0.095 \\
Lemniscate & 0.137 & 0.091 & \textbf{0.085} & 0.100 \\
Lemniscate fast & 0.146 & 0.109 & \textbf{0.108} & - \\
\hline 
Attitude err. [\si{\radian}] & N/c & In-MPC & Post-MPC & D/o \\ 
\hline 
Squares & 0.210 & 0.174 & \textbf{0.167} & - \\
Attitude trajectory & 0.152 & 0.104 & \textbf{0.100} & 0.116\\
Lemniscate & 0.167 & 0.106 & \textbf{0.105} & 0.123\\
Lemniscate fast & 0.215 & \textbf{0.140} & 0.156 & - \\
\hline 
\end{tabular}\caption{Trajectory tracking RMSE of the WMPC approach for different controller configurations and trajectories. N/c = ``No correction'' (i.e., no disturbance compensation).}
\label{tab:trackingWMPC}
\end{table}
% Notes: Experiments used:
% Lemniscate slow: ID 14. 2 reps each, 15s for a single trajectory. Ref. speeds up to 0.9m/s.
% Lemniscate fast: ID 14. 2 reps each, 5.5s for a single trajectory. Ref. speeds up to 2.9m/s
% Attitude trajectory: ID 13, 2 reps each, 27s for a single trajectory.
% Squares: ID 12, 2 reps each. 5s for a single trajectory.

\begin{figure}[ht]
\includegraphics[width=\columnwidth]{plots/13_13_13_13_pos_att_error_comparison.pdf}\caption{Tracking errors of the WMPC during the attitude trajectory for different controller configurations. The violins show the position RMSE on the left (in [\si{\meter}]) and the attitude RMSE on the right (in [\si{\radian}]), respectively.}\label{fig:wmpc_te_violin}
\end{figure}


\subsection{AMPC}
For AMPC, we analyze the influence of the controller tuning (i.e., the actuator input weights) on the pose tracking performance and on the exploitation of the allocation nullspace. To this end, we perform two sets of experiments. In both sets, we first track the reference trajectory with high weights $\weightAlpha$ and then with low weights.
\begin{enumerate*}
    \item We first apply this procedure on the square trajectory. The numerical results in \cref{tab:trackingAMPC} show that the tracking accuracy is higher for high actuator weights.
    \item We then also use this procedure on tracking horizontal position reference steps of \SI{1}{\meter}. Horizontal steps are particularly challenging as they require a sudden thrust direction change that can lead to infeasibly high tilt angle speeds. \Cref{fig:tiltAnglesAMPC} presents the results with a focus on the tilt angle commands. It shows that for low actuator weights, the tilt angle commands change rapidly and exhibit infeasibly high velocities. However, for higher weights, the tilt angle speeds are significantly lower while the position tracking is only slightly affected, resulting in \SI{0.328}{\meter} in the first and \SI{0.351}{\meter} in the latter case, respectively. Furthermore, note the tilt angle drift in the second period. As the weights $\weightAlpha$ are lowered, the allocation nullspace is explored more freely, neglecting the objective to achieve maximum power efficiency.
\end{enumerate*}

% Show deviation of actuator commands from 'optimal' actuator commands
\begin{table}[t!]
\centering
\begin{tabular}{c|c|c|c|c|c}
\hline 
 & $\weightThrust$ & $\weightAlpha$ & $\weightAlphaDot$ & Pos. err. [\si{\meter}] & Att. err. [\si{\radian}]\\ 
\hline 
High alpha cost & 1.0 & 10 & 10 & 0.111 & 0.212 \\
Low alpha cost & 0.1 & 0.1 & 10 & 0.136 & 0.279 \\
\hline 
\end{tabular}\caption{Trajectory tracking RMSE for different controllers and trajectories. For both AMPC tunings, the square trajectory was tracked three times, resulting in evaluation times of \SI{30}{\second}.}
\label{tab:trackingAMPC}
\end{table}
% Info:
% This table has been generated from exp. ID 3.
% For both versions of AMPC, the square trajectory was repeated 3 times


% Experiments: MPC with integrator
% Quality measure: Tracking accuracy
% Compare against: MPC with and without learned model, with and without disturbance observer.


\begin{figure}[ht]
    \includegraphics{plots/21_position_tilt_angles_and_speeds.pdf}
    \caption{Position tracking, tilt angle commands and tilt angle speeds for lateral position steps. The actuator weights are high in the first highlighted period and low in the second highlighted period.}\label{fig:tiltAnglesAMPC}
\end{figure}
% INFO 21:
% Some more jumps, this time with low constraints and also low cost on allocation. Nicely shows how after a few jumps the tilt angles don't come back to the optimal allocation tilt angles. Can see this in plots of tilt angles and of rotor speeds.
% Path: '../kea/mpc/full_actuator/07_27/test4/test4_2021-07-27-09-28-15.bag'
% Trajectories':[[35,62],[83,110]],
% Sets: [[0],'AMPC','AMPC, 1m jumps, alpha_dot_constraint=10,alpha_w=10'],
%       [[1],'AMPC','AMPC, 1m jumps, alpha_dot_constraint=1,alpha_w=0.1']]

% First set of steps (30-70s):
% RMSE Position: [ 0.3189  0.0276  0.0698], norm: 0.327615882099
% RMSE Attitude: [ 0.0523  0.1442  0.0273], norm: 0.155774105032
% Std deviation Position: [ 0.3187  0.0276  0.0453]
% Std deviation Attitude: [ 0.0523  0.1434  0.0273]

% Second set of steps (83-110s):
% RMSE Position: [ 0.3467  0.045   0.026 ], norm: 0.350580368462
% RMSE Attitude: [ 0.0786  0.1612  0.0373], norm: 0.183145772938
% Std deviation Position: [ 0.3467  0.044   0.02  ]
% Std deviation Attitude: [ 0.0762  0.1608  0.0344]


\subsection{Comparison}
Both presented methods have their respective advantages and disadvantages. 
% Implementation, reliability, tuning
\begin{itemize}
    \item Implementation and user-friendliness: Generally, both WMPC and AMPC are similarly complex in their implementation on a flying platform. However, as the input dimensionality of AMPC is considerably larger, tuning weights and constraints can be more tedious as compared to WMPC. Additionally, as AMPC can exploit the entire allocation nullspace of an overactuated vehicle, the flight behavior can be inconsistent and produce non-repeatable results.
    \item Tracking accuracy: Using the Post-MPC formulation in WMPC we have found the highest tracking accuracy. This is due to the no-delay advantage of a learnt model (as opposed to an online filter) and the relatively accurate allocation model at the optimal solution. While AMPC in theory should perform better, we suspect that the combination of longer computation times, the delay produced by the EKF, and the allocation model being inaccurate far away from the optimal solution lead to higher tracking errors.
    \item Power efficiency: As WMPC uses a maximum-power-efficiency allocation, it is more efficient than AMPC, which also produces suboptimal control inputs for the purpose of complying with actuator constraints and the input weights.
    \item Applications: In most applications, WMPC provides a sufficient performance. However, AMPC can be of interest in the case of highly aggressive maneuvers in which actuator constraints need to be considered or in which the optimal allocation solution alone does not produce satisfying results, requiring the exploitation of the allocation nullspace.
    \item Computational complexity: Due to the larger input and state space of AMPC, it takes considerably longer computation times. \Cref{fig:solveTimes} shows that AMPC exceeds the desired computation time of \SI{10}{\milli\second}, especially during periods in which constraints are active. As an example, the second period of \cref{fig:tiltAnglesAMPC} leads to the long solver times of nearly \SI{20}{\milli\second}.% Note: the bump at around 0.02s comes from the second blue period in fig. 7.
\end{itemize}

\begin{figure}[ht]
    \includegraphics{plots/13_21_solve_time_comparison.pdf}
    \caption{Comparison of MPC solver times for WMPC and AMPC.}\label{fig:solveTimes}
\end{figure}

==> arxiv/07_conclusion.tex <==
\section{Conclusion}
We have presented a model predictive control framework for fully actuated or overactuated \acp{MAV}. Within this framework, we have employed two \acp{MPC} that optimize different control inputs and that use different approaches to cope with disturbances that arise from unknown internal effects.

The first one, WMPC, optimizes actuator wrenches which are thereafter translated by an optimal allocation into actuator commands. WMPC can consider disturbances either inside the model formulation (In-MPC) or as a a posteriori correction of the optimal wrench commands (Post-MPC). The disturbances can either be estimated by an EKF or by an approximation through a linear model that is trained on experimental data.

On the other hand, AMPC optimizes actuator commands and relies on an EKF as a disturbance estimator. Due to its knowledge of the actuator allocation, it can exploit the allocation nullspace and direct constraints on actuator commands.

Finally, we have conducted experiments to show the performances of the two controllers and their respective up- and downsides. While the AMPC approach in theory models the system more accurately, it suffers from the higher complexity (both in tuning, repeatability, and in computation). Therefore, the WMPC appraoch remains the preferred method for most use cases.

==> arxiv/acronyms.tex <==

\DeclareAcronym{MAV}{short = MAV, long = micro aerial vehicle}
\DeclareAcronym{AM}{short = AM, long = aerial manipulator}
\DeclareAcronym{COM}{short = CoM, long = center of mass}
\DeclareAcronym{DOF}{short = DoF, long = degrees of freedom}
\DeclareAcronym{NDT}{short = NDT, long = nondestructive testing}
\DeclareAcronym{OMAV}{short = OMAV, long = omnidirectional micro aerial vehicle}
\DeclareAcronym{CAD}{short = CAD, long = computer-aided design}
\DeclareAcronym{IMU}{short = IMU, long = inertial measurement unit}
\DeclareAcronym{TOF}{short = TOF, long = time of flight}
\DeclareAcronym{EKF}{short = EKF, long = extended Kalman filter}
\DeclareAcronym{LQRI}{short = LQRI, long = linear-quadratic regulator with integral action}
\DeclareAcronym{MPC}{short = MPC, long = model predictive control}
\DeclareAcronym{NMPC}{short = NMPC, long = nonlinear model predictive control}
\DeclareAcronym{PID}{short = PID, long = proportional-integral-derivative}
\DeclareAcronym{EE}{short = EE, long = end-effector}
\DeclareAcronym{ROS}{short = ROS, long = Robot Operating System}
\DeclareAcronym{ACADO}{short = ACADO, long = Automatic Control and Dynamic Optimization}
\DeclareAcronym{FT}{short = FT, long = Force-Torque}
\DeclareAcronym{WMPC}{short = WMPC, long = Wrench-MPC}
\DeclareAcronym{AMPC}{short = AMPC, long = Actuator-MPC}
\DeclareAcronym{LBMPC}{short = LBMPC, long = learning-based MPC}



==> arxiv/symbol_definition.tex <==
% ---------- Standard Commands ------------------

\usepackage{color}
\newcommand\red[1]{{\textcolor{red}{#1}}}
\newcommand\blue[1]{{\textcolor{blue}{#1}}}
% ---------- new variables ------------------

\newcommand{\Hinf}{$H_\infty$\xspace}


% ---------- new commands ------------------
\renewcommand{\vec}[1]{\bm{#1}}		% vectors
\newcommand{\mat}[1]{\bm{#1}}		% matrices
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\nR}[1]{\mathbb{R}^{#1}}		% real number
\newcommand{\nN}[1]{\mathbb{N}^{#1}}		% 
\newcommand{\nT}[1]{\mathbb{T}^{#1}}		% real number
\newcommand{\define}{:=}			% define symbol
\newcommand{\abs}[1]{\left| #1 \right|}	% abs
%\newcommand\norm[1]{\left\lVert#1\right\rVert}
\renewcommand{\matrix}[1]{\begin{bmatrix} #1 \end{bmatrix}}	% matrix
\renewcommand{\smallmatrix}[1]{\left[\begin{smallmatrix} #1 \end{smallmatrix}\right]}	% matrix
\newcommand{\cosp}[1]{\cos \left( #1 \right)}	% cos with brace
\newcommand{\sinp}[1]{\sin \left( #1 \right)}	% sin with brace
\newcommand{\determinant}[1]{\text{det}\left(#1\right)} 	% determinant
\newcommand{\sgn}[1]{\text{sgn}\left( #1 \right)}			% signum
\newcommand{\atanTwo}[1]{{\rm atan2}\left( #1\right)}		% atan2
\newcommand{\acotTwo}[1]{{\rm acot2}\left( #1\right)}		% acot2
\newcommand{\upperRomannumeral}[1]{\uppercase\expandafter{\romannumeral#1}}	% roman numbers
\newcommand{\lowerromannumeral}[1]{\romannumeral#1\relax}
% \newcommand{\vSpace}{\;\,}
\newcommand{\transpose}{^\top}
\newcommand{\des}{r}
\newcommand{\desk}{r,k}
\newcommand{\ddt}{\frac{d}{dt}}
\newcommand{\SO}{\mathrm{SO}}
\newcommand{\f}[1]{\prescript{}{#1}{}}

%-----------Functions------------------------
\newcommand{\minEig}[1]{\lambda_{\text{min}}[#1]}
\newcommand{\maxEig}[1]{\lambda_{\text{max}}[#1]}

% --------- References ----------------------
\newcommand{\fig}{Fig.~}	% figure ref
\newcommand{\eqn}{Eq.~}	% equation ref
\newcommand{\tab}{Tab.~}	% table ref
\newcommand{\cha}{Chap.~}	% chapter ref
\newcommand{\sect}{Sec.~}	% section ref

% --------- Variables -----------------------

% General
\renewcommand{\frame}[1]{\mathcal{F}_{#1}}		% frames
\newcommand{\pos}{\vec{p}}				% position vector
\newcommand{\vel}{\vec{v}}				% velocity vector
\newcommand{\rotMat}{\mat{R}}				% rotation matrix
\newcommand{\rotMatVectAngle}[2]{\rotMat_{#1}(#2)}	% rotation matrix representing the rotation about a vector of a certain angle
\newcommand{\vZero}{\vec{0}}				% vect/matr of zeros
\newcommand{\eye}[1]{\mat{I}_{#1}}
\newcommand{\zeros}[1]{\mat{0}_{#1}}

%%%%%%%%%%%%%%%%%%
%% FRAMES
%%%%%%%%%%%%%%%%%%
\newcommand{\body}{{}_B}
\newcommand{\local}{{}_L}
\newcommand{\world}{{}_W}

\newcommand{\origin}{O}
\newcommand{\vX}{\vec{x}}					% x-axis
\newcommand{\vY}{\vec{y}}					% y-axis
\newcommand{\vZ}{\vec{z}}					% z-axis
\newcommand{\vE}[1]{\vec{e}_{#1}}			% standard unit axis

% indices
\newcommand{\meas}{{}_m}

% frame world
\newcommand{\originW}{\origin\world}
\newcommand{\xW}{\vX\world}				% x-axis world frame
\newcommand{\yW}{\vY\world}				% y-axis world frame
\newcommand{\zW}{\vZ\world}				% z-axis world frame

% frame body
\newcommand{\originB}{\origin\body}
\newcommand{\xB}{\vX\body}				% x-axis body frame
\newcommand{\yB}{\vY\body}				% y-axis body frame
\newcommand{\zB}{\vZ\body}				% z-axis body frame

% frame local
\newcommand{\originL}{\origin\local}
\newcommand{\xL}{\vX\local}				% x-axis body frame
\newcommand{\yL}{\vY\local}				% y-axis body frame
\newcommand{\zL}{\vZ\local}				% z-axis body frame

% Rotation matrices
\newcommand{\RB}{\mat{R}_{B}}
\newcommand{\RL}{\mat{R}_{L}}

% States, inputs
\newcommand{\states}{\vec{x}}
\newcommand{\inputs}{\vec{u}}
\newcommand{\stateSpace}{\mathcal{X}}
\newcommand{\inputSpace}{\mathcal{U}}

\newcommand{\roll}{\phi}
\newcommand{\pitch}{\theta}
\newcommand{\yaw}{\psi}
\newcommand{\angAcc}{\dot{\angVel}}		% angular acceleration
\newcommand{\gravity}{\vec{g}}			% gravity vector
\newcommand{\tprop}{t}
\newcommand{\tprops}{\vec{t}}
\newcommand{\tiltangles}{\vec{\alpha}}
\newcommand{\tpropsdot}{\dot{\vec{t}}}
\newcommand{\tiltanglesdot}{\dot{\vec{\alpha}}}

% System
\newcommand{\qB}{\vec{q}}   % Quaternion q_WB
\newcommand{\linAcc}{\vec{a}\body}
\newcommand{\angVel}{\vec{\omega}}		% angular velocity
\newcommand{\eulerAngles}{\vec{\eta}}
\newcommand{\mass}{m}
\newcommand{\inertia}{\bm{J}}
\newcommand{\posDot}{\dot{\pos}}				% position vector
\newcommand{\velDot}{\dot{\vel}}				% velocity vector
\newcommand{\qBDot}{\dot{\qB}}				% velocity vector
\newcommand{\angVelDot}{\dot{\angVel}}				% velocity vector

% controller
\newcommand{\force}{\vec{f}}
\newcommand{\torque}{\vec{\tau}}
\newcommand{\actForce}{\vec{f}_a}
\newcommand{\actTorque}{\vec{\tau}_a}
\newcommand{\actWrench}{\vec{w}_a}
\newcommand{\actWrenchDot}{\dot{\vec{w}}_a}
\newcommand{\actInput}{\inputs_a}
\newcommand{\actInputDot}{\dot{\inputs}_a}
\newcommand{\wrench}{\vec{w}}
\newcommand{\wrenchdot}{\dot{\vec{w}}}

% Disturbance and disturbance estimate:
\newcommand{\torquecom}{\torque_{\text{com}}}

% \newcommand{\rCOM}{\vec{r}_{\text{com}}}
% \newcommand{\rBT}{\vec{r}_T}

% IMU measurement data:
\newcommand{\imuLinAccMeas}{\vec{a}_{IMU}}
\newcommand{\imuLinBias}{\vec{a}_b}
\newcommand{\imuLinNoise}{\vec{a}_n}
\newcommand{\imuAngAccMeas}{\dot{\vec{\omega}}_{IMU}}
\newcommand{\imuAngVel}{\vec{\omega}_{IMU}}
\newcommand{\imuAngVelBias}{\vec{\omega}_b}
\newcommand{\imuAngVelNoise}{\vec{\omega}_n}
\newcommand{\imuAngAcc}{\dot{\vec{\omega}}_{IMU}}

% Model learning
\newcommand{\features}{\tilde{\vec{x}}}
%\newcommand{\featuresMean}{\bar{\vec{x}}}
\newcommand{\modelMatrix}{\mat{C}}
\newcommand{\outputs}{\vec{y}}
\newcommand{\outputsMean}{\bar{\vec{y}}}

\newcommand{\tiltAngle}{\alpha}
\newcommand{\tiltAngles}{\vec{\alpha}}
\newcommand{\dtiltAngles}{\dot{\vec{\alpha}}}
\newcommand{\rotorSpeed}{\omega}
\newcommand{\rotorSpeeds}{\vec{\omega}}
\newcommand{\drotorSpeeds}{\dot{\vec{\omega}}}
\newcommand{\thrustComponents}{\tilde{\vec{t}}}

\newcommand{\nrot}{n_r}
\newcommand{\nrotperarm}{n_{rpa}}
\newcommand{\narms}{n_a}

% ALLOCATION:
\newcommand{\allocationMatrix}{\mat{A}}

% MPC:
\newcommand{\qErr}{\vec{q}_{\text{e}}}
\newcommand{\qErrk}{\vec{q}_{\text{e},k}}
\newcommand{\RBdes}{\mat{R}_{B,\des}}
\newcommand{\discreteDynamics}{\vec{g}}
\newcommand{\stageCost}{\vec{h}}

\newcommand{\nstates}{n}
\newcommand{\ninputs}{m}
\newcommand{\nfeatures}{n_f}
\newcommand{\nsamples}{n_s}

% ESTIMATOR:
\newcommand{\stateEst}{\hat{\vec{x}}}
\newcommand{\posEst}{\hat{\pos}}
\newcommand{\velEst}{\hat{\vel}}
\newcommand{\qBEst}{\hat{\qB}}
\newcommand{\ekfInputs}{\vec{u}_{EKF}}
\newcommand{\ekfMeasurements}{\vec{z}_{EKF}}
\newcommand{\posMeas}{\pos\meas}
\newcommand{\qBMeas}{\qB\meas}
\newcommand{\distTorqueEst}{\Delta\hat{\torque}}
\newcommand{\distForceEst}{\Delta\hat{\force}_L}
\newcommand{\angVelEst}{\hat{\vec{\omega}}}		% angular velocity
\newcommand{\processNoise}{\vec{n}}

% MODEL LEARNING:
\newcommand{\torqueResidual}{\Delta\torque}
\newcommand{\torqueResidualMeasured}{\Delta\torque\meas}
\newcommand{\forceResidual}{\Delta\force}
\newcommand{\forceResidualEst}{\Delta\hat{\force}}
\newcommand{\forceResidualMeasured}{\Delta\force\meas}
\newcommand{\forceResidualLocal}{\Delta\force_L}
\newcommand{\distForceLocal}{\forceResidualLocal}
\newcommand{\wrenchResidual}{\Delta\wrench}
\newcommand{\wrenchResidualMeasured}{\Delta\wrench\meas}
\newcommand{\wrenchResidualModel}{\Delta\bar{\wrench}}
\newcommand{\distTorque}{\Delta\torque}
\newcommand{\trainError}{\vec{e}_{train}}
\newcommand{\params}{\vec{c}}
\newcommand{\featureMatrix}{\mat{X}}
\newcommand{\regParam}{\lambda}

% FULL ACTUATOR MPC:
\newcommand{\weightThrust}{w_T}
\newcommand{\weightAlpha}{w_\alpha}
\newcommand{\weightAlphaDot}{w_{\dot{\alpha}}}
\newcommand{\mpcStateWeights}{\mat{Q}}
\newcommand{\mpcInputWeights}{\mat{R}}
\newcommand{\actForceConstraint}{f_{a,max}}
\newcommand{\actTorqueConstraint}{\tau_{a,max}}
\newcommand{\actWrenchConstraint}{\wrench_{a,max}}
\newcommand{\actWrenchDotConstraint}{\dot{\wrench}_{a,max}}
\newcommand{\tpropsMin}{\vec{t}_{min}}
\newcommand{\tpropsMax}{\vec{t}_{max}}


\DeclareSIUnit{\amperehour}{Ah}
